Calibrating Self-supervised Monocular Depth Estimation

In the recent years, many methods demonstrated the ability of neural networks to learn depth and pose changes in a sequence of images, using only self-supervision as the training signal. Whilst the networks achieve good performance, the often over-looked detail is that due to the inherent ambiguity of monocular vision they predict depth up to an unknown scaling factor. The scaling factor is then typically obtained from the LiDAR ground truth at test time, which severely limits practical applications of these methods. In this paper, we show that incorporating prior information about the camera configuration and the environment, we can remove the scale ambiguity and predict depth directly, still using the self-supervised formulation and not relying on any additional sensors.

==> scratch.tex <==

% Similar to other self-supervised depth detection networks we approach the problem using two subnetworks: one for depth of a single image $D_t=\phi(I_t)$ on the image $I_t$, another for pose change between two images $P_{(t, t+i)} = \rho(I_t, I_{t+i})$. The function $\omega$ then takes $I_t, D_t, P_{(t, t+i)}$ and the camera instrinsics $K$ and warps $I_t$ to the viewpoint of $I_{t+i}$, we write this as: $\Hat{I_{t+i}} = \omega(I_t, D_t, P_{(t, t+i)}, K)$.\\
% We then compare these two images using a combination of
% \begin{equation}
%     L^1(\Hat{I_t+i}, I_{t+i})  = ||(\Hat{I_t+i} - I_{t+i})||
% \end{equation}
% and

% \begin{equation}
%     SSIM(\Hat{I_{t+i}}, I_{t+i})=\frac{(2\mu_{I_{t+i}}\mu_{\Hat{I_{t+i}}}+c_1)(2\sigma_{\Hat{I_{t+i}} I_{t+i}}+c_2)}{(\mu^2_{L_{t+i}}+\mu_{\Hat{L_{t+i}}}^2+c_1)(\sigma_{L_{t+i}}^2+\sigma_{\Hat{L_{t+i}}}^2+c_2})
% \end{equation}


% where $\mu_x$ is the mean of $x$, $\sigma_x^2$ is the variance of $x$ and $\sigma_{xy}$ is the covariance of $x$ and $y$.\\

% Similar to \cite{monodepthv2} we apply a mask on photometric losses to remove stationary pixels which is defined as
% \begin{equation}
%     \mu = [ \min_i E_p(I_{t}, I_{t+i}) < \min_i E_p(I_{t}, \hat{I_{t+i}})]
% \end{equation}
% where $[]$ is the Iverson bracket which created a binary mask in pixel space. $\mu$ therefore ignores the loss of pixels where the reprojection error of the unwarped source image $I_{t+i}$ is lower than the warped image $\hat{I_{t+i}}$\\
% We combine these loss functions in the following equation which we minimize:
% \begin{equation}
%     E_p(\hat{I_{t+i}}, I_{t+i}) = \sum_i (\alpha \frac{1-SSIM(\hat{I_{t+i}}, I_{t+i})}{2} + (1-\alpha)L^1(\hat{I_{t+i}}, I_{t+i}))[\mu]
% \end{equation}
% where $\alpha =0.85$ and $[\mu]$ masks images.

% without additionally having a LiDAR sensor on-board. Current methods at test time apply a scaling using the median value of LiDAR points which are also captured by the image using the following equation:
% \begin{equation}
%     mask = LiDAR > 0\\
% \end{equation}
% \begin{equation}
%     prediction =prediction \times  \frac{median(LiDAR[mask])} {median(prediction[mask])}
%     \label{eq:lidar_scaling}
% \end{equation}
% Where $prediction$ is the output of our network (inverted as we predict inverse depth) and $LiDAR$ is an image of sparse LiDAR points projected into an image with the same viewpoint as our input image, $mask$ indicates indices where sparse LiDAR points are captured and $LiDAR[mask]$ gives an array of these values.

==> tables/weight_ablation.tex <==
\begin{table}[!t]
  \centering
  \caption{Weighting applied to new loss}
%   \vspace{-10pt}
  \resizebox{\textwidth}{!}{
  \begin{tabular}{|c|c|c|c|c|c|c|c|c|}
  \hline
  Steps  & \cellcolor{col1}Abs Rel & \cellcolor{col1}Sq Rel & \cellcolor{col1}RMSE  & \cellcolor{col1}RMSE log & \cellcolor{col2}$\delta < 1.25 $ & \cellcolor{col2}$\delta < 1.25^{2}$ & \cellcolor{col2}$\delta < 1.25^{3}$\\
  
  \hline
  
 
0.1 & 0.148 & 1.041 & 5.343 & 0.234 & 0.783 & 0.943 & 0.976 \\
0.125 & 0.132 & 0.996 & 5.109 & 0.214 & 0.827 & 0.95 & 0.978 \\
0.15 & 0.131 & 1.003 & 5.067 & 0.209 & 0.837 & 0.953 & 0.979 \\
0.175 & 0.132 & 0.988 & 5.029 & 0.207 & 0.842 & 0.953 & 0.98 \\
0.2 & 0.134 & 1.005 & 5.058 & 0.208 & 0.842 & 0.954 & 0.98 \\
0.225 & 0.142 & 1.055 & 5.12 & 0.21 & 0.838 & 0.952 & 0.98 \\
0.25 & 0.146 & 1.079 & 5.154 & 0.21 & 0.837 & 0.953 & 0.981 \\
0.275 & 0.15 & 1.144 & 5.26 & 0.212 & 0.831 & 0.951 & 0.98 \\
0.3 & 0.151 & 1.147 & 5.213 & 0.212 & 0.833 & 0.952 & 0.98 \\
0.4 & 0.159 & 1.159 & 5.248 & 0.216 & 0.823 & 0.952 & 0.981 \\
0.5 & 0.178 & 1.283 & 5.432 & 0.224 & 0.795 & 0.951 & 0.981 \\
0.6 & 0.178 & 1.317 & 5.526 & 0.225 & 0.798 & 0.949 & 0.981 \\


\arrayrulecolor{black}\hline

  \end{tabular}
  }%\hfill
\label{tab:weights}  
% \vspace{-10pt}
\end{table}

